MERGETUNE: Continued Fine-Tuning of Vision-Language Models

Fine-tuning vision-language models (VLMs) such as CLIP often leads to catastrophic forgetting of pretrained knowledge. Prior work primarily aims to mitigate forgetting during adaptation; however, forgetting often remains inevitable during this process. We introduce a novel paradigm, continued fine-tuning (CFT), which seeks to recover pretrained knowledge after a zero-shot model has already been adapted. We propose a simple, model-agnostic CFT strategy (named MERGETUNE) guided by linear mode connectivity (LMC), which can be applied post hoc to existing fine-tuned models without requiring architectural changes. Given a fine-tuned model, we continue fine-tuning its trainable parameters (e.g., soft prompts or linear heads) to search for a continued model which has two low-loss paths to the zero-shot (e.g., CLIP) and the fine-tuned (e.g., CoOp) solutions. By exploiting the geometry of the loss landscape, the continued model implicitly merges the two solutions, restoring pretrained knowledge lost in the fine-tuned counterpart. A challenge is that the vanilla LMC constraint requires data replay from the pretraining task. We approximate this constraint for the zero-shot model via a second-order surrogate, eliminating the need for large-scale data replay. Experiments show that MERGETUNE improves the harmonic mean of CoOp by +5.6% on base-novel generalisation without adding parameters. On robust fine-tuning evaluations, the LMC-merged model from MERGETUNE surpasses ensemble baselines with lower inference cost, achieving further gains and state-of-the-art results when ensembled with the zero-shot model. Our code is available at https://github.com/Surrey-UP-Lab/MERGETUNE.

==> sec/statement.tex <==
\subsection{Ethics statement}
This work focuses on methodological improvements for adapting vision-language models and does not involve the collection of new human subject data. All datasets used in our experiments are publicly available, widely adopted in prior research, and contain images and annotations curated for academic use. We follow the same usage protocols as the original dataset authors and cite the relevant sources. As our method builds on pretrained models such as CLIP, potential biases or societal impacts inherited from these models may still be present in downstream applications. We encourage careful consideration of these risks when deploying our approach in real-world systems.



\subsection{Reproducibility statement}
We ensure reproducibility by providing comprehensive details of our experimental setup. The datasets, model architectures, and baselines we use are all publicly available. Our training configurations, including hyperparameters and optimization settings, are described in the main paper and supplement. To further support replication, we include our code in the supplementary material. In addition, we perform multiple runs with different random seeds and report averaged results to ensure statistical robustness.
